Combining Deep Reinforcement Learning and Search for Imperfect-Information Games

The combination of deep reinforcement learning and search at both training and test time is a powerful paradigm that has led to a number of successes in single-agent settings and perfect-information games, best exemplified by AlphaZero. However, prior algorithms of this form cannot cope with imperfect-information games. This paper presents ReBeL, a general framework for self-play reinforcement learning and search that provably converges to a Nash equilibrium in any two-player zero-sum game. In the simpler setting of perfect-information games, ReBeL reduces to an algorithm similar to AlphaZero. Results in two different imperfect-information games show ReBeL converges to an approximate Nash equilibrium. We also show ReBeL achieves superhuman performance in heads-up no-limit Texas hold'em poker, while using far less domain knowledge than any prior poker AI.

==> core/A0_value_functions.tex <==
\section{Value Functions}
\label{sec:value_functions}

Let $\mathbb{K}$ represent the set of joint belief states (JB states) (i.e., a joint probability distribution over world states in a public state). We would like to have a function $V$ that takes as input a JB state $\beta$ and a belief state $b$, and outputs a 

Let $b$ represent a belief state (that is, a probability distribution over the world states in an information set). There exists (in theory) a value function which takes as input $b_1, b_2$ and outputs a matrix $A$ of values for pairs of hands, given the belief distributions $b_1$,$b_2$. That is, the entry of matrix $A_{2\spadesuit 2\heartsuit,K\diamondsuit K\clubsuit}$ is the value of player~$1$ holding $2\spadesuit 2\heartsuit$ when player~$2$ is holding $K\diamondsuit K\clubsuit$ given the beliefs $b_1,b_2$. Since there are ${52 \choose 2} = 1326$ possible hands, $A$ is a $1326 \times 1326$ matrix (though due to card removal, not all of the entries are relevant). It's difficult to learn the output of a $1326 \times 1326$ matrix directly, but fortunately we don't need to. We only need $b_2 A$.

We would like to have a value function (which we assume WLOG is for player~$1$) that takes as input $b_{ave,1},b_{ave,2},b_{curr,2}$ and outputs a value for each hand 
$V_1(b_{ave,1},b_{ave,2},b_{curr,2}) = \vec{v}_1 = [v_1(2\spadesuit2\heartsuit),v_1(2\spadesuit2\diamondsuit),...,v_1(A\diamondsuit A\clubsuit)] = $

==> core/A1_dvalue.tex <==
\section{Derivation of algorithm based on $dV/dB$}

A set of joint beliefs at a game node defines a subgame $G(B)$. We'll say that $V(h_0, h_1|\pi)$ is the value of a particular initial state (hands $h_0$ and $h_1$) in this subgame, assuming players play according to strategy $\pi$. Let $\pi^*_{G(B)}$ be a Nash equilibrium strategy for $G(B)$.

The value of a hand $h_0$ at a leaf node with beliefs $B^b$, assuming Nash equilibrium play according to beliefs $B^f$ from that point onwards, is

\begin{align}
V_0(h_0 | B^f, B^b) = \sum_{h_1} { V(h_0, h_1 | \pi^*_{G(B^f)}) B^b(h_1) }
\end{align}

(we will call $B^f$ and $B^b$ the forward and backward beliefs, respectively).

During CFR, $V_0(h_0 | B, B)$ can be substituted for the value of a subset of nodes, and CFR will still converge to Nash for all nodes that are not descendants of those nodes (DeepStack).

In fact, CFR will still converge if $V_0(h_0 | B_{avg}, B)$ is used, where we use $B_{avg}$, the beliefs implied by the average strategy up to the node, as the forward beliefs (see Theorem~\ref{th:cfrd}).

Suppose we have a model $\hat{V}_0(h_0|B) = V_0(h_0 | B, B) + \epsilon(B)$, where $\epsilon(B)$ is an error term.

\begin{align}
    \frac{d}{dB} \hat{V}_0(h_0|B) = \frac{d}{dB^f} V_0(h_0|B^f, B)|_{B^f=B} + \frac{d}{dB^b} V_0(h_0|B, B^b)|_{B^b=B} + \frac{d}{dB} \epsilon(B)
\end{align}

The RHS has three terms, lets consider them individually.

For the first term, notice

\begin{align}
    \frac{d}{dB^f} V_0(h_0|B^f, B)|_{B^f=B} = \frac{d V_0(h_0|B^f, B)|_{B^f=B}}{d\pi^*_{G(B^f)}} \cdot \frac{d\pi^*_{G(B^f)}}{dB^f} 
\end{align}

Consider the meaning of these two terms. The first term is the change in the value of hand $h_0$ as the policy $\pi^*_{G(B^f)}$ changes, while the second term is the change in equilibrium policy as a function of beliefs. The first term $dV/d\pi$ must be 0 for any direction on the simplex, because otherwise the gradient $dV/d\pi$ would be a direction that The direction of the second term must be on the simplex, and by the definition of $\pi^*$ as an equilibrium policy, it

==> core/A3_jointbelief_proof.tex <==
\section{Proof of Theorem~\ref{th:jbstate}}
\begin{proof}
Let $K$ be a CK set. Let $s \in K$ be a world state in $K$ and let $I_i$ be the infostate containing $s$ for player~$i$. $\rho(s) = \rho_c(s) \Pi_{i \in \mathcal{P}} \rho_i(s)$. Since $\rho_i(s) = \rho_i(I_1)$ so $\rho(s) = \rho_c(s) \Pi_{i \in \mathcal{P}} \rho_i(I_i)$. The probability $\rho_c(s)$ is a fixed quantity determined from the rules of the game.

Thus, $\rho(s)$ can be computed given only $\rho_i(I_i)$ for each player $i$, and the rules of the game.
\end{proof}


==> core/A4_common_knowledge.tex <==
\section{Extension to Common Knowledge Sets}
\label{sec:ck}

==> core/A6_exit_values.tex <==
\section{Safety via Selection of a Random Iteration's Policy}

This section explains in more detail why our algorithm chooses a \emph{random} iteration's policy at test time rather than the policy on the final iteration or the average policy over all iterations. As an example of the problem our approach is designed to address, consider again the game of modified Rock-Paper-Scissors as illustrated in Figure~\ref{fig:app_rps1} and Figure~\ref{fig:app_rps2} where the optimal policy is to choose Rock and Paper with probability $0.4$ and Scissors with probability $0.2$.

\begin{figure}[!h]
	\vspace{-0.15in}
	\centering
	\begin{subfigure}[t!]{.48\textwidth}
		\centering
		\includegraphics[width=65mm]{figures/new_rps1.pdf}
		\vspace{-0.2in}
		\caption{Variant of Rock-Paper-Scissors in which the optimal $P_1$ policy is (R=0.4, P=0.4, S=0.2). Terminal values are color-coded. The dotted lines mean $P_2$ does not know which node they are in.}
		\label{fig:app_rps1}
	\end{subfigure}%
	\quad
	\begin{subfigure}[t!]{.48\textwidth}
		\centering
		\includegraphics[width=65mm]{figures/new_rps2.pdf}
		\vspace{-0.2in}
		\caption{The $P_1$ subgame when using perfect-information one-ply lookahead search. Leaf values are determined by the full-game equilibrium. There is insufficient information for finding (R=0.4, P=0.4, S=0.2).}
		\label{fig:app_rps2}
	\end{subfigure}
\end{figure}

As a start, let's suppose that we have perfectly learned the value function $\hat{v}$ and are now playing against a real opponent where we are $P_2$ and the opponent is $P_1$.

The most intuitive algorithm, which we refer to as \textbf{unsafe} search, is to first run CFR for $T$ iterations for $P_1$'s first move (for some large fixed $T$) and eventually arrive at a policy such as $(R = 0.401, P = 0.399, S = 0.2)$. We pass down the beliefs resulting from that policy, and now compute our optimal policy as $P_2$. This would result in a policy of $(R = 0, P = 1, S = 0)$ for $P_2$. This is clearly not a Nash equilibrium. Moreover, if our opponent knew we would end up playing this policy (which we assume they would know since we assume they know the algorithm we run to generate the policy), then they could counter us by playing $(R = 0, P = 0, S = 1)$.

This problem demonstrates the need for \textbf{safe} search, which is a search algorithm that ensures we play a Nash equilibrium policy in expectation. Importantly, it is \emph{not} necessary for the policy that the algorithm outputs to always be a Nash equilibrium. It is only necessary that the algorithm outputs a Nash equilibrium policy \emph{in expectation}. For example, in modified Rock Paper Scissors it is acceptable for an algorithm to output a policy of 100\% Rock, so long as the probability it outputs that policy is~40\%.

There have been several prior papers on how to do safe search in imperfect-information games~\cite{burch2014solving,moravcik2016refining,brown2017safe,moravvcik2017deepstack}. All past approaches to safe search involve knowing (or estimating) the value of each opponent infostate in the subgame.
Such an approach to safe search presents major issues, especially for a self-play algorithm. For one, the value network is what we are training during self-play, and the existing safe search algorithms are not guaranteed to improve the value network. Thus, we would either have to use the value network only some of the time during training (which would make the algorithm much more expensive), or only do safe search at test time. But doing safe search at test time when it was not used during training could potentially lead to PBSs that were not encountered during training time and therefore that our value network is not trained to handle.

Our approach to safe search is to run the exact same algorithm that was used during training: we pick a random iteration and play according to the policy on that iteration. This leads to a PBS leaf node, which defines a new subgame, and the process repeats. Theorem~\ref{th:safe}, the proof of which is in Section~\ref{sec:proof_safe}, states that this algorithm approximates a Nash equilibrium.
